Oracle inequalities and minimax rates for non-local means and related adaptive kernel-based methods

This paper describes a novel theoretical characterization of the performance of non-local means (NLM) for noise removal. NLM has proven effective in a variety of empirical studies, but little is understood fundamentally about how it performs relative to classical methods based on wavelets or how various parameters (e.g., patch size) should be chosen. For cartoon images and images which may contain thin features and regular textures, the error decay rates of NLM are derived and compared with those of linear filtering, oracle estimators, variable-bandwidth kernel methods, Yaroslavsky's filter and wavelet thresholding estimators. The trade-off between global and local search for matching patches is examined, and the bias reduction associated with the local polynomial regression version of NLM is analyzed. The theoretical results are validated via simulations for 2D images corrupted by additive white Gaussian noise.

==> Im_YF0_100_barbara.tex <==
\renewcommand{\currentcaption}{YF0, MSE = 8.45e+02}
\renewcommand{\currentname}{Im_YF0_100_barbara}


==> notations.tex <==

\newcommand{\currentcaption}{}
\newcommand{\currentname}{}

\newcommand{\joefig}[2]{\input{./latex_figures/#2}  \subfigure[\currentcaption]{\includegraphics[width=#1\linewidth]{\currentname}}}



%SHORT CUTS:
\newcommand{\nc}{\newcommand}

% Image
\newcommand{\inoisy}{\mathbf Y} 
\newcommand{\itrue}{\mathbf f}
\newcommand{\patch}{\textsf{P}}
%\newcommand{\wnlm}[2]{\omega ( #1 , #2 )}
\newcommand{\wnlm}{\omega}


\makeatletter

\newcommand*{\wpatch}{%
 \protect \@ifnextchar\bgroup\w@patch\w@@patch
}

\newcommand*{\w@patch}[1]{% Commande exécutée si une accolade ouvrante est détectée.
  \ensuremath{\boldsymbol S \left( #1 \right)}%
}

\newcommand*{\w@@patch}{% Commande exécutée si aucune accolade ouvrante n’est détectée.
  \ensuremath{\boldsymbol S}%
}

\newcommand*{\wpatchoppose}{%
 \protect \@ifnextchar\bgroup\my@patch\my@@patch
}

\newcommand*{\my@patch}[1]{% Commande exécutée si une accolade ouvrante est détectée.
  \ensuremath{\check{(\boldsymbol S}\left( #1 \right)}%
}

\newcommand*{\my@@patch}{% Commande exécutée si aucune accolade ouvrante n’est détectée.
  \ensuremath{\check{\boldsymbol S}}%
}


\makeatother


\newcommand{\boldx}{ x}
\newcommand{\ihat}{\hat{\itrue}}
\newcommand{\divs}{\mathbf D}

\newcommand{\norm}[2][]{{\left \lVert #2 \right\rVert}_{#1}}

%SETS
\newcommand{\R}{\mathbb{R}}
\newcommand{\A}{\mathbb{A}}
\newcommand{\B}{\mathbb{B}}
\newcommand{\N}{\mathbb{N}}
%\newcommand{\L}{\mathbb{L}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\G}{\mathbb{G}}
\newcommand{\D}{\mathbb{D}}
%\newcommand{\H}{\mathbb{H}}
\newcommand{\I}{\mathbb{I}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}

% PROBA
\nc{\ind}{\mathds{1}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\V}{\mathbb{V}\mbox{ar}\,}
\newcommand{\vt}{\mbox{Var}_\theta\,}
\newcommand{\ct}{\mbox{Cov}_\theta\,}


% classe de fonctions
\DeclareMathOperator{\PSNR}{PSNR}
\DeclareMathOperator{\MSE}{MSE}
\DeclareMathOperator{\FMSE}{FMSE}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Cor}{Cor}
\DeclareMathOperator{\Cov}{Cov}

%\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\Mixt}{Mixt}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\Sp}{Sp}
%\DeclareMathOperator{\Range}{Range}
\DeclareMathOperator{\DST}{\mathcal D}
\DeclareMathOperator{\ols}{OLS}

\DeclareMathOperator{\cls}{CLS}
\DeclareMathOperator{\NAIVECLS}{Naive-CLS}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%                  NOTATION SHORTCUTS FOR ESTIMATORS ETC....          %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 

\newcommand{\alphaBF}{\mathbf{\alpha}} 
\newcommand{\hatfMRE}{\hat{\mathbf{f}}_{\text{\tiny MRE}}} 
\newcommand{\hatfLIN}{\hat{\mathbf{f}}_{\text{\tiny LIN}}} 
\newcommand{\hatfUNIF}{\hat{\mathbf{f}}_{\text{\tiny UWA}}} 
\newcommand{\hatfCVX}{\hat{\mathbf{f}}_{\text{\tiny CVX}}} 

\newcommand{\divergence}{\text{div}}
\newcommand{\hatr}{\boldsymbol{r}}
\newcommand{\hatrlbd}{\hatr_{\lambda}}
\newcommand{\hatrEWA}{\hat{r}_\text{\tiny EWA}} 
\newcommand{\AEWA}{{A}_\text{\tiny EWA}} 
\newcommand{\hatf}{\hat{\mathbf{f}}}
\newcommand{\hatfWAV}{\hat{\mathbf{f}}_\text{\tiny WAV}}
\newcommand{\hatfEWA}{\hat{\mathbf{f}}_\text{\tiny EWA}}
\newcommand{\hatfEWAi}{\hat{\mathbf{f}}_{\text{\tiny EWA},i}} 
\newcommand{\albd}{A_{\lambda}}
\newcommand{\albdo}{A_{\lambda_0}}
\newcommand{\blbd}{b_{\lambda}} 
\newcommand{\flbd}{f_{\lambda}}
\newcommand{\hatflbd}{\hatf_{\lambda}}
\newcommand{\hatflbdi}{\hatf_{\lambda,i}} 
\newcommand{\hatflbdo}{\hatf_{\lambda_0}}
\newcommand{\ymoinsflbd}{\| \YY - \hatflbd \|^2_n}
\newcommand{\ymoinshatf}{\| \YY - \hatf \|^2_n}
\newcommand{\ymoinshatfEWA}{\| \YY - \hatfEWA \|^2_n} 
\newcommand{\ymoinsf}{\| Y - f \|^2_n}
\newcommand{\ttlbd}{\theta(\lambda)}
\newcommand{\pilbd}{\pi(\lambda)}
\newcommand{\intlbd}{\int_{\Lambda}}
\newcommand{\gradrlbd}{\nabla \hatrlbd}
\newcommand{\YY}{\boldsymbol Y}
\newcommand{\ssigma}{\boldsymbol\sigma}
\newcommand{\In}{I_{n\times n}}
\newcommand{\calPlbd}{\mathcal{P}_\Lambda}
\newcommand{\KL}{\mathcal{K}}
\newcommand{\1}{\mathds{1}}





%% Ery shortcuts




% environments
\newtheorem{thm}{Theorem}[section]
%\newtheorem{thm}{Theorem}
\newtheorem{prp}{Proposition}[section]
\newtheorem{lem}{Lemma}[section]
\newtheorem{cor}{Corollary}[section]
%\newtheorem{definition}{Definition}[section]

\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqn}{\begin{eqnarray*}}
\newcommand{\eeqn}{\end{eqnarray*}}
\newcommand{\bitem}{\begin{itemize}}
\newcommand{\eitem}{\end{itemize}}
\newcommand{\benum}{\begin{enumerate}}
\newcommand{\eenum}{\end{enumerate}}
\newcommand{\bmult}{\begin{multline*}}
\newcommand{\emult}{\end{multline*}}
\newcommand{\bcenter}{\begin{center}}
\newcommand{\ecenter}{\end{center}}

% references
\newcommand{\thmref}[1]{Theorem~\ref{thm:#1}}
\newcommand{\prpref}[1]{Proposition~\ref{prp:#1}}
%\renewcommand{\corref}[1]{Corollary~\ref{cor:#1}}
\newcommand{\lemref}[1]{Lemma~\ref{lem:#1}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
%\newcommand{\newcommand{ref}[1]{Definition~\ref{def:#1}}

% operators
\nc{\argmin}{\mathop{\mathrm{arg\,min}}}
\nc{\argmax}{\mathop{\mathrm{arg\,max}}}

%\DeclareMathOperator{\det}{det}
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\dist}{dist}
%\DeclareMathOperator{\rank}{rank}
%\DeclareMathOperator{\span}{span}
\DeclareMathOperator{\trace}{trace}
\DeclareMathOperator{\tr}{tr}
%\DeclareMathOperator{\diag}{diag}

% functions
\DeclareMathOperator{\acos}{acos}
\DeclareMathOperator{\asin}{asin}
\DeclareMathOperator{\atan}{atan}

% cal letters
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

% bold letters (upper case)
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\bO}{\mathbf{O}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}

% bold letters (lower case)
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\bbf}{\mathbf{f}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bh}{\mathbf{h}}
\newcommand{\bi}{\mathbf{i}}
\newcommand{\bj}{\mathbf{j}}
\newcommand{\bk}{\mathbf{k}}
\newcommand{\bl}{\mathbf{l}}
\newcommand{\bm}{\mathbf{m}}
\newcommand{\bn}{\mathbf{n}}
\newcommand{\bo}{\mathbf{o}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bt}{\mathbf{t}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}

% bold greek letters
\newcommand{\bbeta}{{\boldsymbol\beta}}
\newcommand{\bmu}{{\boldsymbol\mu}}
\newcommand{\bxi}{{\boldsymbol\xi}}
\newcommand{\btheta}{{\boldsymbol\theta}}
\newcommand\bSigma{{\boldsymbol\Sigma}}
\newcommand\bOmega{{\boldsymbol\Omega}}
\newcommand{\beps}{{\boldsymbol\eps}}

% bb letters
\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbH}{\mathbb{H}}
%\newcommand{\bbI{\mathbb{I}}
\newcommand{\bbI}{\mathds{1}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbO}{\mathbb{O}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bbY}{\mathbb{Y}}
\newcommand{\bbZ}{\mathbb{Z}}

% probability

\newcommand{\expect}[1]{\mathbb{E}\left(#1\right)}
\newcommand{\pr}[1]{\mathbb{P}\left(#1\right)}
\newcommand{\var}[1]{\operatorname{Var}\left(#1\right)}
\newcommand{\cov}[1]{\operatorname{Cov}\left(#1\right)}
%\newcommand{\cor}[1]{\operatorname{Cor}\left(#1\right)}

% \newcommand\indep{\protect\mathpalette{\protect\independenT}{\perp}}
% \newcommand{\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

\newcommand{\iid}{\stackrel{\rm iid}{\sim}}
\newcommand{\Bin}{\text{Bin}}
\newcommand{\Unif}{\text{Unif}}
\newcommand{\lsto}{\stackrel{\rm sto}{\leq}}
\newcommand{\gsto}{\stackrel{\rm sto}{\geq}}

% other symbols
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
\newcommand{\inner}[2]{\langle #1, #2 \rangle}
\newcommand{\ang}[2]{\angle \left(#1, #2\right)}
\newcommand{\eps}{\varepsilon}
%\newcommand{\implies}{\ \Rightarrow \ }
%\newcommand{\iff}{\ \Leftrightarrow \ }
\DeclareMathOperator{\sign}{sign}
\newcommand{\Vol}{{\rm Vol}}

% anotation
\definecolor{darkgreen}{rgb}{.0,.638,.035}
\definecolor{darkred}{rgb}{.638,.0,.035}
\definecolor{purple}{rgb}{0.4,.1,.9}
\newcommand{\eac}[1]{\textcolor{purple}{(Ery: #1)}}
\newcommand{\ery}[1]{\textcolor{purple}{#1}}
\newcommand{\joe}[1]{\textcolor{red}{Joe: #1}}
\newcommand{\jrs}[1]{\textcolor{red}{#1}}
\newcommand{\becca}[1]{\textcolor{darkgreen}{(Becca: #1)}}
\newcommand{\bmw}[1]{\textcolor{darkgreen}{#1}}

% other
\newcommand{\mse}{{\rm MSE}}
\newcommand{\ie}{{\em i.e.,~}}
\newcommand{\eg}{{\em e.g.,~}}
\newcommand{\lcf}{{\em cf.\ }}

\newcommand{\pix}{{\rm pix}}
\newcommand{\ave}{{\rm Ave}}
\newcommand{\one}[1]{\mathds{1}_{\{ #1 \}}}
\newcommand{\fin}{f_\Omega}
\newcommand{\fout}{f_{\Omega^c}}
\newcommand{\gin}{g_\Omega}
\newcommand{\gout}{g_{\Omega^c}}
\newcommand{\afloor}{\lfloor \alpha \rfloor}
%\newcommand{\NLMm}{$\overline{\rm NLM}$}
\newcommand{\NLMm}{NLM-average}
\newcommand{\poly}{{\rm poly}}
\newcommand{\cf}{C_0}
\newcommand{\wh}[1]{\widehat{#1}}
\renewcommand{\mp}{{m_\patch}}
\newcommand{\byp}{{\by_\patch}}
\newcommand{\bypi}{{\by_{\patch_i}}}
\newcommand{\bypj}{{\by_{\patch_j}}}
\newcommand{\bep}{{\beps_\patch}}
\newcommand{\bepi}{{\beps_{\patch_i}}}
\newcommand{\bepj}{{\beps_{\patch_j}}}
\newcommand{\bbfp}{{\bbf_\patch}}
\newcommand{\bbfpi}{{\bbf_{\patch_i}}}
\newcommand{\bbfpj}{{\bbf_{\patch_j}}}
%\newcommand{\ypbar}{{\overline{\yp}}}
%\newcommand{\epbar}{{\overline{\ep}}}
\newcommand{\ypbar}{{\overline{\byp}}}
\newcommand{\fpbar}{{\overline{\bbfp}}}
\newcommand{\epbar}{{\overline{\bep}}}

%\newcommand{\ypbari}{{\overline{\bypi}}}
%\newcommand{\fpbari}{{\overline{\bbfpi}}}
%\newcommand{\epbari}{{\overline{\bepi}}}
%
%\newcommand{\ypbarj}{{\overline{\bypj}}}
%\newcommand{\fpbarj}{{\overline{\bbfpj}}}
%\newcommand{\epbarj}{{\overline{\bepj}}}

\newcommand{\ypbark}{{\overline{y}_{\patch_k}}}
\newcommand{\ypbari}{{\overline{y}_{\patch_i}}}
\newcommand{\fpbari}{{\overline{f}_{\patch_i}}}
\newcommand{\epbari}{{\overline{\eps}_{\patch_i}}}

\newcommand{\ypbarj}{{\overline{y}_{\patch_j}}}
\newcommand{\fpbarj}{{\overline{f}_{\patch_j}}}
\newcommand{\epbarj}{{\overline{\eps}_{\patch_j}}}


